On the dimension of limit sets on $\mathbb{P}(\mathbb{R}^3)$ via stationary measures: variational principles and applications

In this article, we establish the variational principle of the affinity exponent of Borel Anosov representations. We also establish such a principle of the Rauzy gasket. In Li-Pan-Xu, they obtain a dimension formula of the stationary measures on $\mathbb{P}(\mathbb{R}^3)$. Combined with our result, it allows us to study the Hausdorff dimension of limit sets of Anosov representations in $\mathrm{SL}_3(\mathbb{R})$ and the Rauzy gasket. It yields the equality between the Hausdorff dimensions and the affinity exponents in both settings. In the appendix, we improve the numerical lower bound of the Hausdorff dimension of Rauzy gasket to $1.5$.

==> macros.tex <==
\RequirePackage{extarrows}
\RequirePackage{mathtools}
\RequirePackage{textcomp}
\RequirePackage{wasysym}
\RequirePackage{tikz}
\RequirePackage{graphicx}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usepackage{esint}
\usepackage[T1]{fontenc}

\newcommand{\highlight}[1]{{\color{magenta} #1}}
\newcommand{\significant}[1]{\textbf{\color{red} #1}}

% 统一
\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand\LHS{\mathrm{LHS}}
\newcommand\RHS{\mathrm{RHS}}
%\newcommand\cd{\, \bm\cdot\, }
\newcommand\defeq{\coloneqq}

\numberwithin{equation}{section}
\newcommand{\case}[1]{\left\{\begin{aligned}
#1
\end{aligned}\right.}

% Brackets
\newcommand{\lb}[1]{\left\{#1\right\}}
\newcommand{\mb}[1]{\left[#1\right]}
\renewcommand{\sb}[1]{\left(#1 \right)}
\newcommand{\msb}[1]{\left[#1\right)}
\newcommand{\smb}[1]{\left(#1 \right]}

\newcommand{\bsb}[1]{\big(#1\big)}
\newcommand{\Bsb}[1]{\Big(#1\Big)}
\newcommand{\bbsb}[1]{\bigg(#1\bigg)}
\newcommand{\BBsb}[1]{\Bigg(#1\Bigg)}


% 一些缩写
\newcommand{\vp}{\varphi}
\newcommand{\ve}{\varepsilon}
\newcommand{\vk}{\varkappa}
\newcommand{\vn}{\varnothing}
\newcommand{\sbs}{\subset}
\newcommand{\sbse}{\subseteq}
\newcommand{\sps}{\supset}
\newcommand{\spse}{\supseteq}
\newcommand{\sm}{\setminus}
\newcommand{\ag}[1]{\begin{aligned}#1\end{aligned}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}


% 分析
\DeclareMathOperator{\Ran}{\mathrm{Range}}
\DeclareMathOperator{\supp}{\mathrm{supp}}
\DeclareMathOperator{\Rl}{\mathrm{Re}}
\DeclareMathOperator{\Img}{\mathrm{Im}}
\DeclareMathOperator{\Lip}{\mathrm{Lip}}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\pv}{p.v.}
\DeclareMathOperator{\Spec}{\mathrm{Spec}}
\renewcommand{\ae}[1][]{\ #1\mathrm{a.e.}\ }
%\newcommand{\one}{\bm{\mathbbm 1}}
\newcommand\D{\mathrm D}
\newcommand\dr{\mathrm{d}}
\newcommand{\Leb}{\mathrm{Leb}}
\newcommand{\pa}{\partial^\alpha}

\newcommand{\nm}[1]{\left\|#1\right\|}
\newcommand{\gnm}[1]{\recbracket#1\recbracket}
\newcommand{\dv}[2][0]{\left.\frac{\dr}{\dr #2}\right|_{#2=#1}}
\newcommand{\pt}[2][]{\frac{\partial#1}{\partial #2}}%partial
\newcommand{\tv}[2]{\left. #1\right|_{#2}}%take values


\newcommand{\lto}[1]{\stackrel{#1}{\longrightarrow}}
\newcommand{\pair}[1]{\left\langle#1\right\rangle}
\newcommand{\abs}[1]{\left|#1\right|}

% 动力系统
\DeclareMathOperator{\Prob}{\mathrm{Prob}}
\newcommand{\Diff}{\mathrm{Diff}}
\newcommand{\Homeo}{\mathrm{Homeo}}
\newcommand{\gr}{\mathrm{gr}}
\newcommand{\Orb}{\mathrm{Orb}}
\newcommand{\reg}{\mathrm{reg}}

% 几何群论
\DeclareMathOperator{\Cay}{\mathrm{Cay}}
\DeclareMathOperator{\Ax}{\mathrm{Ax}}

% 概率
\DeclareMathOperator{\var}{var}
%\renewcommand{\P}{\bm{\mathrm P}}

% 代数与数论
\DeclareMathOperator{\spaned}{\mathrm{span}}
\DeclareMathOperator{\Tr}{\mathrm{tr}}
\DeclareMathOperator{\rank}{\mathrm{rank}}
\renewcommand{\mod}{\ \mathrm{mod}\ }
\newcommand{\Ad}{\mathrm{Ad}}
\newcommand{\ad}{\mathrm{ad}}
\newcommand\lcm{\mathrm{lcm}}
\newcommand{\Aut}{\mathrm{Aut}}
\newcommand{\End}{\mathrm{End}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\Isom}{\mathrm{Isom}}

\newcommand{\GL}{\mathrm{GL}}
\newcommand{\SL}{\mathrm{SL}}
\newcommand{\PSL}{\mathrm{PSL}}
\newcommand{\SO}{\mathrm{SO}}

\newcommand{\mtx}[1]{\footnotesize{\mb{\setlength{\arraycolsep}{2.5pt}\begin{matrix}#1\end{matrix}}}}
\DeclareMathOperator{\Cl}{\mathrm{Cl}}

% 几何
\DeclareMathOperator{\Ind}{\mathrm{Ind}}
\newcommand{\Vol}{\mathrm{Vol}}
\DeclareMathOperator{\diam}{\mathrm{diam}}



% \mathcal字体
\newcommand{\cA}{\mathcal A}
\newcommand{\cB}{\mathcal B}
\newcommand{\cC}{\mathcal C}
\newcommand{\cD}{\mathcal D}
\newcommand{\cE}{\mathcal E}
\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}
\newcommand{\cH}{\mathcal H}
\newcommand{\cI}{\mathcal I}
\newcommand{\cJ}{\mathcal J}
\newcommand{\cK}{\mathcal K}
\newcommand{\cL}{\mathcal L}
\newcommand{\cM}{\mathcal M}
\newcommand{\cN}{\mathcal N}
\newcommand{\cO}{\mathcal O}
\newcommand{\cP}{\mathcal P}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\cR}{\mathcal R}
\newcommand{\cS}{\mathcal S}
\newcommand{\cT}{\mathcal T}
\newcommand{\cU}{\mathcal U}
\newcommand{\cV}{\mathcal V}
\newcommand{\cW}{\mathcal W}
\newcommand{\cX}{\mathcal X}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cZ}{\mathcal Z}

% \mathscr字体
\newcommand{\sA}{\mathscr A}
\newcommand{\sB}{\mathscr B}
\newcommand{\sC}{\mathscr C}
\newcommand{\sD}{\mathscr D}
\newcommand{\sE}{\mathscr E}
\newcommand{\sF}{\mathscr F}
\newcommand{\sG}{\mathscr G}
\newcommand{\sH}{\mathscr H}
\newcommand{\sI}{\mathscr I}
\newcommand{\sJ}{\mathscr J}
\newcommand{\sK}{\mathscr K}
\newcommand{\sL}{\mathscr L}
\newcommand{\sM}{\mathscr N}
\newcommand{\sN}{\mathscr N}
\newcommand{\sO}{\mathscr O}
\newcommand{\sP}{\mathscr P}
\newcommand{\sQ}{\mathscr Q}
\newcommand{\sR}{\mathscr R}
\newcommand{\sS}{\mathscr S}
\newcommand{\sT}{\mathscr T}
\newcommand{\sU}{\mathscr U}
\newcommand{\sV}{\mathscr V}
\newcommand{\sW}{\mathscr W}
\newcommand{\sX}{\mathscr X}
\newcommand{\sY}{\mathscr Y}
\newcommand{\sZ}{\mathscr Z}



% \mathbb 字体
\renewcommand{\AA}{{\mathbb A}}
\newcommand{\BB}{{\mathbb B}}
\newcommand{\CC}{{\mathbb C}}
\newcommand{\DD}{{\mathbb D}}
\newcommand{\EE}{{\mathbb E}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\GG}{{\mathbb G}}
\newcommand{\HH}{{\mathbb H}}
\newcommand{\II}{{\mathbb I}}
\newcommand{\JJ}{{\mathbb J}}
\newcommand{\KK}{{\mathbb K}}
\newcommand{\LL}{{\mathbb L}}
\newcommand{\MM}{{\mathbb M}}
\newcommand{\NN}{{\mathbb N}}
\newcommand{\OO}{{\mathbb O}}
\newcommand{\PP}{{\mathbb P}}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\RR}{{\mathbb R}}
\renewcommand{\SS}{{\mathbb S}}
\newcommand{\TT}{{\mathbb T}}
\newcommand{\UU}{{\mathbb U}}
\newcommand{\VV}{{\mathbb V}}
\newcommand{\WW}{{\mathbb W}}
\newcommand{\XX}{{\mathbb X}}
\newcommand{\YY}{{\mathbb Y}}
\newcommand{\ZZ}{{\mathbb Z}}


% 黑体
\newcommand{\bA}{{\mathbf{A}}}
\newcommand{\bB}{{\mathbf{B}}}
\newcommand{\bC}{{\mathbf{C}}}
\newcommand{\bD}{{\mathbf{D}}}
\newcommand{\bE}{{\mathbf{E}}}
\newcommand{\bF}{{\mathbf{F}}}
\newcommand{\bG}{{\mathbf{G}}}
\newcommand{\bH}{{\mathbf{H}}}
\newcommand{\bI}{{\mathbf{I}}}
\newcommand{\bJ}{{\mathbf{J}}}
\newcommand{\bK}{{\mathbf{K}}}
\newcommand{\bL}{{\mathbf{L}}}
\newcommand{\bM}{{\mathbf{M}}}
\newcommand{\bN}{{\mathbf{N}}}
\newcommand{\bO}{{\mathbf{O}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\bQ}{{\mathbf{Q}}}
\newcommand{\bR}{{\mathbf{R}}}
\newcommand{\bS}{{\mathbf{S}}}
\newcommand{\bT}{{\mathbf{T}}}
\newcommand{\bU}{{\mathbf{U}}}
\newcommand{\bV}{{\mathbf{V}}}
\newcommand{\bW}{{\mathbf{W}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\bY}{{\mathbf{Y}}}
\newcommand{\bZ}{{\mathbf{Z}}}






% 一些哥特体
\newcommand{\fh}{\mathfrak h}
\newcommand{\fg}{\mathfrak g}
\newcommand{\fu}{\mathfrak u}
\newcommand{\fo}{\mathfrak o}
\newcommand{\fr}{\mathfrak r}
\newcommand{\fsu}{\mathfrak{su}}
\newcommand{\fgl}{\mathfrak{gl}}
\newcommand{\fsl}{\mathfrak{sl}}
\newcommand{\fsp}{\mathfrak{sp}}
\newcommand{\fso}{\mathfrak{so}}
\newcommand{\ft}{\mathfrak t}
\newcommand{\fz}{\mathfrak z}
\newcommand{\fs}{\mathfrak s}
\newcommand{\fM}{\mathfrak M}





\newcommand{\recbracket}{
\,
\begin{tikzpicture}[baseline]
\draw (0,-0.2em) -- (0em,0.8em) -- (0.2em,0.8em) -- (0.2em,-0.2em) -- (-0.02em,-0.2em);
\end{tikzpicture}
\,
}
\newcommand{\act}{
\,
\tikzset{every picture/.style={line width=0.07em}}
\begin{tikzpicture}[baseline]
\draw  (0,0) .. controls (0,0.8em) and (0.5em,0.8em) .. (0.5em,0);
\draw  (0.65em,0.15em) .. controls (0.56em,0.1em) and (0.52em,0.05em) .. (0.5em,0) .. controls (0.48em,0.05em) and (0.44em,0.1em) .. (0.35em,0.15em);
\end{tikzpicture}
\,
}

% WH use
%\newcommand{\dd}{\,\mathrm{d}}
\newcommand{\hFur}{h_\mathrm{F}}   % Furstenberg entropy
\newcommand{\hRW}{h_\mathrm{RW}}   % Random walk entropy
\newcommand{\dimH}{\dim_\mathrm{H}}% Hausdorff dimension
\newcommand{\unif}{u}     % uniform measure
\newcommand{\Zmodd}{[d]}           % Z mod d Z
\newcommand{\CCs}{\pi_0}             % Connected components
\newcommand{\len}[1]{\lvert#1\rvert}
\DeclareMathOperator{\Stab}{Stab}
\DeclareMathOperator{\Fix}{Fix}
\DeclareMathOperator{\st}{st}      % cancellation
\DeclareMathOperator{\cl}{cl}      % cancellation
\DeclareMathOperator{\lcp}{lcp}      % longest common prefix


\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}




%LPX use
\renewcommand{\bf}[1]{\mathbf{#1}}
\renewcommand{\rm}[1]{\mathrm{#1}}
\renewcommand{\cal}[1]{\mathcal{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\renewcommand{\frak}[1]{\mathfrak{#1}}
\newcommand{\bm}[1]{\mathbbm{#1}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\olive}[1]{{\color{olive}#1}}
\newcommand{\teal}[1]{{\color{teal}#1}}

\def\R{\bb R}
\def\C{\bb C}
\def\P{\bb P}
\def\T{\bb T}
\def\B{\mathbbm 1}
\def\Z{\bb Z}
\def\Q{\bb Q}
\def\S{\bb S}
\def\N{\bb N}
\def\H{\bb H}
\def\E{\bb E}

\def\calA{\cal A}
\def\calQ{\cal Q}
\def\calJ{\cal J}
\def\calF{\cal F}
\def\calO{\cal O}
\def\diag{\rm{diag}}
%\def\diam{\rm{diam}}
\def\SL{\rm{SL}}
\def\PGL{\rm{PGL}}
\def\PSL{\rm{PSL}}
\def\GL{\rm{GL}}
\def\SO{\rm{SO}}
\def\Id{\rm{Id}}
\def\Hom{\rm{Hom}}
\def\HA{\rm{HA}}

\def\bi{\bf i}
\def\bj{\bf j}
%\def\bU{\mathbf{U}}
%\def\bI{\mathbf{I}}

%\DeclareMathOperator{\arccot}{\rm{arccot}}
%\DeclareMathOperator{\sech}{\rm{sech}}
%\newcommand{\supp}{\rm{supp}}

%补丁
\renewcommand{\ve}{\epsilon}


























